Fixation times on directed graphs

Computing the rate of evolution in spatially structured populations is difficult. A key quantity is the fixation time of a single mutant with relative reproduction rate $r$ which invades a population of residents. We say that the fixation time is "fast" if it is at most a polynomial function in terms of the population size $N$. Here we study fixation times of advantageous mutants ($r>1$) and neutral mutants ($r=1$) on directed graphs, which are those graphs that have at least some one-way connections. We obtain three main results. First, we prove that for any directed graph the fixation time is fast, provided that $r$ is sufficiently large. Second, we construct an efficient algorithm that gives an upper bound for the fixation time for any graph and any $r\ge 1$. Third, we identify a broad class of directed graphs with fast fixation times for any $r\ge 1$. This class includes previously studied amplifiers of selection, such as Superstars and Metafunnels. We also show that on some graphs the fixation time is not a monotonically declining function of $r$; in particular, neutral fixation can occur faster than fixation for small selective advantages.

==> theorems/common.tex <==



What follows is an adaptation of Theorem 6 of \cite{diaz2013fixation}
and Theorem 1 of \cite{he2001drift} to be applied to
the case of advantageous mutants in the Moran birth-death
process.

\begin{theorem}[Theorem 6 of \cite{diaz2014approximating}]\label{thm:diaz-drift-theorem}
Let $(Y_t)_{t\geq 0}$ be a Markov chain with state space $\Omega$,
where $Y_0$ is chosen from some set $I \subseteq \Omega$.
If there are constants $k_1, k_2 > 0$
and a non-negative function $\psi\colon \Omega \to\Real$ such that
\begin{itemize}
    \item $\psi(S) = 0$ for some $S \in \Omega$,
    \item $\psi(S) \leq k_1$ for all $S \in I$, and
    \item $\mathbb E[\psi(Y_t) - \psi(Y_{t+1}) | Y_t = S] \geq k_2$
    for all $t \geq 0$
    and all $S$ with $\psi(S) > 0$,
\end{itemize}
    then $\mathbb E[\tau] \leq k_1/k_2$, where $\tau := \min \{t : \psi(Y_t) = 0\}$.
\end{theorem}
\begin{proof}
    See the proof of Theorem 6 from \cite{diaz2014approximating}.
\end{proof}

% \begin{lemma}[Time until minimum is reached, minimum is only possible absorbing state, strictly decreasing drift]\label{lemma:drift-first-moment}
%     Let $\mathscr{X} \equiv (X_t)_{t\geq0}$ be a Markov chain from the state space
%     $\Omega$.
%     Suppose $\psi\colon\Omega\to[0,1]$ is such that
%     \begin{enumerate}
%         \item $\psi(S) = 0$ for some $S\in\Omega$ and
%         \item there is some $\e > 0$ with
%             $\E{\psi(X_{t})-\psi(X_{t+1})\mid X_t=S} \geq \e$
%             for each $t\geq 0$ and
%             for each $S\in\Omega$ with $\psi(S)>0$.
%     \end{enumerate}
%     Let $\tau := \min\Set{t\geq0\mid \psi(X_t)=0}$.
%     Then
%     \begin{equation}
%         \E{\tau} \leq \frac{\psi(X_0)}{\e}.
%     \end{equation}
% \end{lemma}

\begin{lemma}[Time until maximum is reached, maximum is only possible absorbing state, strictly increasing drift]\label{lemma:drift-first-moment-upwards}
    Let $\mathscr{X} \equiv (X_t)_{t\geq0}$ be a Markov chain from the state space
    $\Omega$.
    Suppose $\mu\colon\Omega\to[0,1]$ is such that
    \begin{enumerate}
        \item $\mu(S) = 1$ for some $S\in\Omega$ and
        \item there is some $\e > 0$ with
            $\E{\mu(X_{t+1})-\mu(X_{t})\mid X_t=S} \geq \e$
            for each $t\geq 0$ and
            for each $S\in\Omega$ with $\mu(S)<1$.
    \end{enumerate}
    Let $\tau := \min\Set{t\geq0\mid \mu(X_t)=1}$
    and $\kappa := \sup\Set{k \in [0,1] \mid \Pr[\mu(X_0)<k] = 0}$.
    Then
    \begin{equation}
        \E{\tau} \leq \frac{1-\kappa}{\e}.
    \end{equation}
\end{lemma}
\begin{proof}
    Take $\psi \equiv 1-\mu$, $Y_t = X_t$, $I$ as the support of $X_0$,
    $k_1 = 1-\kappa$, and $k_2 = \e$.
    Then the result follows from \cref{thm:diaz-drift-theorem}.
\end{proof}

% \begin{lemma}\label{lemma:modified-moran}
%     Let $M'_r$ be like the Moran process $M_r$ with relative fitness $r\geq 1$ on a graph
%     except that on extinction, a single mutant is placed at the
%     initial mutant location (this counts as an extra time step).
%     Then the expected fixation time of $M_r$ is at most the expected absorption time of $M'_r$.
% \end{lemma}
% \begin{proof}
%     For $M'_r$, consider the last time $t$ there are no mutants in the population.
%     Since the process only uses the immediate last state to generate its current state, $M'_r$ from time $t+1$ has the same
%     distribution as $M_r$ when $M_r$ is conditioned on fixation occurring.
%     Thus the expected fixation time of $M_r$ is equal to the
%     expected absorption time of $M'_r$ minus $t+1$, which is upper bounded by the expected absorption time of $M'_r$.
% \end{proof}

\begin{lemma}\label{lemma:modified-moran}
    Let $M'_r$ be like the Moran process $M_r$ with relative fitness $r\geq 1$ on a graph
    except that on extinction, a single mutant is placed at the
    initial mutant location (this counts as an extra time step).
    Then the expected absorption time of $M_r$ is at most the expected absorption time of $M'_r$.
\end{lemma}
% \begin{proof}
%     % For $M'_r$, consider the last time $t$ there are no mutants in the population.
%     % Since the process only uses the immediate last state to generate its current state, $M'_r$ from time $t+1$ has the same
%     % distribution as $M_r$ when $M_r$ is conditioned on fixation occurring.
%     % Thus the expected fixation time of $M_r$ is equal to the
%     % expected absorption time of $M'_r$ minus $t+1$, which is upper bounded by the expected absorption time of $M'_r$.
% \end{proof}

\begin{lemma}\label{lemma:abs-to-fix}
    Let $M_r$ be a Moran process with mutants that have relative fitness $r\geq 1$.
    Let $\AT_r$, $\FT_r$, and $\ET_r$ be the
    (unconditional) expected absorption time, the expected absorption time conditional on fixation (i.e. fixation time),
    and the expected absorption time conditioned on extinction (i.e. extinction time), respectively.
    Let $\fpminr$ denote the minimum fixation probability of $M_r$ across all non-empty initial mutant placements.
    Then
    \begin{equation}
        \FT_r \leq \AT_r / \fpminr
    \end{equation}
\end{lemma}
\begin{proof}
    For any initial mutant configuration
    we have $\AT_r = \FT_r\cdot \fp^{(r)} + \ET_r\cdot (1-\fp^{(r)})$.
    Then we know $\ET_r\cdot (1-\fp^{(r)})\geq 0$, thus $\AT_r\geq \FT_r\fp^{(r)}$.
    Finally, we have $\fp^{(r)}\geq \fpminr$.
\end{proof}

% \begin{proof}
%     For any time $t\geq 1$ by the total law of expectation
%     \begin{equation}
%         \E{\mu(X_t)\mid X_0}
%         = \E{\E{\mu(X_{t-1}) + (\mu(X_t)-\mu(X_{t-1}))\mid X_{t-1}}\mid X_0}
%     \end{equation}
%     and by linearity of expectation
%     \begin{equation}
%        \E{\mu(X_{t-1}) + (\mu(X_t)-\mu(X_{t-1}))\mid X_{t-1}} 
%        \geq \E{\mu(X_{t-1})\mid X_{t-1}} + \e
%        = \mu(X_{t-1}) + \e.
%     \end{equation}
%     By induction on $t$
%     \begin{equation}
%         \E{\mu(X_t)\mid X_0}
%         \geq \E{\mu(X_{t-1}) + \e\mid X_0}
%         \geq \E{\mu(X_{0}) + t\e\mid X_0}
%         = \mu(X_{0}) + \E{t\e\mid X_0}.
%     \end{equation}
%     We know that $\mu(\mathscr{X})$ is a sub-martingale since by linearity of expectation,
%     \begin{equation}
%         \E{\mu(X_{t+1})\mid X_t} \geq \E{\mu(X_t)\mid X_t} + \e
%         \geq \mu(X_t)
%     \end{equation}
%     for each $t\geq0$.
%     Since $\tau$ is finite, we get
%     \begin{equation}
%         \lim_{t\to\infty}\E{\mu(X_t)\mid X_0} = p.
%     \end{equation}
%     
%     % Then since $\mathscr{X}$ is a discrete-time sub-martingale, there must
%     % exists some time $t^*$ such that $\E{\mu(X_{t^*})\mid X_0}=1$
%     % and $\E{\mu(X_t)\mid X_0}<1$ for all $t<t^*$.
%     % Notice that $\tau = t^*$ by definition.
%     
%     Finally we have
%     \begin{equation}
%         1 = \E{\mu(X_\tau)\mid X_0}
%         \geq \mu(X_0) + \E{\tau\e\mid X_0}
%         =\mu(X_0) + \e\cdot\E{\tau\mid X_0}.
%     \end{equation}
%     Rearranging the terms gives the claim.
% \end{proof}


% DO we need these?

\begin{lemma}\label{lemma:drift-variance}
    Let $\mathscr{X} \equiv (X_t)_{t\geq0}$ be a Markov chain from the state space
    $\Omega$.
    Suppose $\mu$ is probability measure on $\Omega$ such that % there is some
    % $\eta > 0$ with
    $\E{\mu(X_{t+1})\mid X_t}\geq\mu(X_t)$ for each $t\geq 0$.
    % and $\Var{\mu(X_{t+1}) \mid X_t}\geq \eta$ for each $t\geq 0$.
    %Let $\tau = \inf\Set{t\geq0\mid \mu(X_t)\in \Set{0,1}}$.
    Let $Y_t := \frac12\cdot\mu(X_t)(1+\mu(X_t))$ for each $t\geq 0$.
    Then
    \begin{equation}
        \E{Y_{t+1}-Y_t\mid X_t} \geq \frac12\cdot\Var{\mu(X_{t+1})\mid X_t}
    \end{equation}
    for all $t\geq0$.
    % \begin{equation}
    %     \E{\tau\mid X_0} \leq \frac{\mu(X_0)(1-\mu(X_0))}{\eta}.
    % \end{equation}
\end{lemma}
% \begin{proof}
%     See Corollary 26 of \cite{kotzing2019first} for the inspiration.
%     We have
%     \begin{align}
%             2\cdot\E{Y_{t+1}-Y_t\mid X_t} 
%          &=  \left(\E{\mu(X_{t+1})\mid X_t}+\E{\mu(X_{t+1})^2\mid X_t}\right)-\left(\mu(X_t)+\mu(X_t)^2\right) \\
%          &=  \left(\E{\mu(X_{t+1})\mid X_t}-\mu(X_t)\right)+\left(\E{\mu(X_{t+1})^2\mid X_t}-\mu(X_t)^2\right) \\
%          &\geq \E{\mu(X_{t+1})^2\mid X_t}-\mu(X_t)^2 \\
%          &\geq \E{\mu(X_{t+1})^2\mid X_t}-\left(\E{\mu(X_{t+1})\mid X_t}\right)^2 \\
%          &= \Var{\mu(X_{t+1})\mid X_t}.
%     \end{align}
% \end{proof}

\begin{lemma}[Absorption time for non-negative drift]\label{lemma:drift-second-moment}
    Let $\mathscr{X} \equiv (X_t)_{t\geq0}$ be a Markov chain from the state space
    $\Omega$ with $X_0\neq\emptyset$.
    Suppose $\mu$ is probability measure on $\Omega$ such that there is some
    $\eta > 0$ with
    $\E{\mu(X_{t+1})\mid X_t} \geq \mu(X_t)$ and $\Var{\mu(X_{t+1})\mid X_t}\geq \eta$ for each $t\geq 0$ with $X_t \not\in\Set{\emptyset,\Omega}$.
    Let $\tau = \inf\Set{t\geq0\mid \mu(X_t)=1}$.
    Then
    \begin{equation}
        \E{\tau\mid X_0} \leq \frac{1-\mu(X_0)(1+\mu(X_0))}{\eta/2}.
    \end{equation}
\end{lemma}
% \begin{proof}
%     This follows from Lemmas \ref{lemma:drift-first-moment} and \ref{lemma:drift-variance}.
% \end{proof}

\begin{lemma}\label{lemma:drift-variance-exactly-zero}
    Let $\mathscr{X} \equiv (X_t)_{t\geq0}$ be a Markov chain from the state space
    $\Omega$.
    Suppose $\mu$ is probability measure on $\Omega$ such that % there is some
    % $\eta > 0$ with
    $\E{\mu(X_{t+1})\mid X_t}=\mu(X_t)$ for each $t\geq 0$.
    % and $\Var{\mu(X_{t+1}) \mid X_t}\geq \eta$ for each $t\geq 0$.
    %Let $\tau = \inf\Set{t\geq0\mid \mu(X_t)\in \Set{0,1}}$.
    Let $Y_t := 1-\mu(X_t)(1-\mu(X_t))$ for each $t\geq 0$.
    Then
    \begin{equation}
        \E{Y_{t+1}-Y_t\mid X_t} = \Var{\mu(X_{t+1})\mid X_t}
    \end{equation}
    for all $t\geq0$.
    % \begin{equation}
    %     \E{\tau\mid X_0} \leq \frac{\mu(X_0)(1-\mu(X_0))}{\eta}.
    % \end{equation}
\end{lemma}
% \begin{proof}
%     This is similar to the proof of Lemma \ref{lemma:drift-variance}.
%     We have
%     \begin{align}
%             \cdot\E{Y_{t+1}-Y_t\mid X_t} 
%          &=  \left(\mu(X_t)-\mu(X_t)^2\right)-\left(\E{\mu(X_{t+1})\mid X_t}-\E{\mu(X_{t+1})^2\mid X_t}\right) \\
%          &=  \left(\E{\mu(X_{t+1})^2\mid X_t}-\mu(X_t)^2\right)-\left(\E{\mu(X_{t+1})\mid X_t}-\mu(X_t)\right) \\
%          &= \E{\mu(X_{t+1})^2\mid X_t}-\mu(X_t)^2 \\
%          &= \E{\mu(X_{t+1})^2\mid X_t}-\left(\E{\mu(X_{t+1})\mid X_t}\right)^2 \\
%          &= \Var{\mu(X_{t+1})\mid X_t}.
%     \end{align}
% \end{proof}

\begin{lemma}[Absorption time for zero drift]\label{lemma:drift-second-moment-exactly-zero}
    Let $\mathscr{X} \equiv (X_t)_{t\geq0}$ be a Markov chain from the state space
    $\Omega$.
    Suppose $\mu$ is probability measure on $\Omega$ such that there is some
    $\eta > 0$ with
    $\E{\mu(X_{t+1})\mid X_t} = \mu(X_t)$ and $\Var{\mu(X_{t+1})\mid X_t}\geq \eta$ for each $t\geq 0$.
    Let $\tau = \inf\Set{t\geq0\mid \mu(X_t)\in\Set{0,1}}$.
    Then
    \begin{equation}
        \E{\tau\mid X_0} \leq \frac{\mu(X_0)(1-\mu(X_0))}{\eta}.
    \end{equation}
\end{lemma}
% \begin{proof}
%     This follows from Lemmas \ref{lemma:drift-first-moment} and \ref{lemma:drift-variance-exactly-zero}.
% \end{proof}

\begin{lemma}[Naive variance lower bound]\label{lemma:variance-lower-bound}
    Let $\mathscr{X} \equiv (X_t)_{t\geq0}$ be a Markov chain from the state space
    $\Omega$.
    For each $t\geq0$, let $\Event_t$ be the event $\mu(X_{t+1}) < \mu(X_t)$.
    Suppose $\mu$ is probability measure on $\Omega$ such that % there is some
    % $\eta > 0$ with
    $\E{\mu(X_{t+1})\mid X_t}\geq\mu(X_t)$
    with
    $\Pr[\Event_t | X_t] \geq \nu_t$ 
    and, given $\Event_t$, $|\mu(X_{t+1})-\mu(X_t)|\geq \ell_t$
    for each $t\geq 0$.
    Then
    \begin{equation}
        \Var{\mu(X_{t+1})\mid X_t} \geq \left(\nu_t\ell_t\right)^2
    \end{equation}
    for all $t\geq0$ with $X_t \not\in\Set{\emptyset,\Omega}$.
\end{lemma}
% \begin{proof}
%     We have
%     \begin{align}
%          \Var{\mu(X_{t+1})\mid X_t}
%          &= \E{\left(\mu(X_{t+1})-\E{\mu(X_{t+1})\mid X_t}\right)^2\mid X_t} \\
%          &\geq \left(\E{\big|\mu(X_{t+1})-\E{\mu(X_{t+1})\mid X_t}\big|\mid X_t}\right)^2
%     \end{align}
%     by Jensen's inequality.
%     Then 
%     \begin{align}
%         \E{\big|\mu(X_{t+1})-\E{\mu(X_{t+1})\mid X_t}\big|\mid X_t}
%         &\geq \nu_t \cdot \ell_t
%     \end{align}
%     since the expectation is non-negative and $\mu(\mathscr X)$ is a submartingale.
% \end{proof}


\begin{lemma}[Naive variance lower bound, zero drift]\label{lemma:variance-lower-bound-zero-drift}
    Let $\mathscr{X} \equiv (X_t)_{t\geq0}$ be a Markov chain from the state space
    $\Omega$.
    For each $t\geq0$, let $\Event_t$ be the event $\mu(X_{t+1}) \neq \mu(X_t)$.
    Suppose $\mu$ is probability measure on $\Omega$ such that 
    $\E{\mu(X_{t+1})\mid X_t}=\mu(X_t)$
    with
    $\Pr[\Event_t | X_t] \geq \nu_t$ 
    and, given $\Event_t$, $|\mu(X_{t+1})-\mu(X_t)|\geq \ell_t$
    for each $t\geq 0$.
    Then
    \begin{equation}
        \Var{\mu(X_{t+1})\mid X_t} \geq \left(\nu_t \ell_t\right)^2
    \end{equation}
    for all $t\geq0$ with $X_t \not\in\Set{\emptyset,\Omega}$.
\end{lemma}
% \begin{proof}
%     We have
%     \begin{align}
%          \Var{\mu(X_{t+1})\mid X_t}
%          &= \E{\left(\mu(X_{t+1})-\E{\mu(X_{t+1})\mid X_t}\right)^2\mid X_t} \\
%          &= \E{\left(\mu(X_{t+1})-\mu(X_{t})\right)^2\mid X_t} \\
%          &\geq \left(\E{\big|\mu(X_{t+1})-\mu(X_{t})\big|\mid X_t}\right)^2
%     \end{align}
%     by Jensen's inequality.
%     Then 
%     \begin{align}
%        \E{\big|\mu(X_{t+1})-\mu(X_{t})\big|\mid X_t}
%         &\geq \nu_t \ell_t
%     \end{align}
%     since the expectation is non-negative and $\mu(\mathscr X)$ is a martingale.
% \end{proof}





% \begin{lemma}[Special variance lower bound]\label{lemma:special-variance-lower-bound}
%     Let $\mathscr{X} \equiv (X_t)_{t\geq0}$ be a Markov chain from the state space
%     $\Omega$.
%     For each $t\geq0$, let $\Event_t$ be the event $\mu(X_{t+1}) > \mu(X_t)$.
%     Suppose $\mu$ is probability measure on $\Omega$ such that % there is some
%     % $\eta > 0$ with
%     $\E{\mu(X_{t+1})\mid X_t}\geq\mu(X_t)$
%     with
%     $\Pr[\Event_t | X_t] \geq \nu_t$ 
%     and, given $\Event_t$, $|\mu(X_{t+1})-\mu(X_t)|\geq \ell_t$
%     for each $t\geq 0$.
%     Further, suppose that for each $t\geq0$ when $\Event_t$ occurs we have $\mu(X_{t+1})\geq \E{\mu(X_{t+1})\mid X_t}$.
%     Then
%     \begin{equation}
%         \Var{\mu(X_{t+1})\mid X_t} \geq \left(\nu_t\ell_t\right)^2
%     \end{equation}
%     for all $t\geq0$ with $X_t \not\in\Set{\emptyset,\Omega}$.
% \end{lemma}
% \begin{proof}
%     We have
%     \begin{align}
%          \Var{\mu(X_{t+1})\mid X_t}
%          &= \E{\left(\mu(X_{t+1})-\E{\mu(X_{t+1})\mid X_t}\right)^2\mid X_t} \\
%          &\geq \left(\E{\big|\mu(X_{t+1})-\E{\mu(X_{t+1})\mid X_t}\big|\mid X_t}\right)^2
%     \end{align}
%     by Jensen's inequality.
%     Then 
%     \begin{align}
%         \E{\big|\mu(X_{t+1})-\E{\mu(X_{t+1})\mid X_t}\big|\mid X_t,\Event_t}
%         &\geq \E{\big|\mu(X_{t+1})-\mu(X_t)\big|\mid X_t,\Event_t}
%         \geq \ell_t.
%     \end{align}
%     Therefore 
%         \begin{align}
%         \E{\big|\mu(X_{t+1})-\E{\mu(X_{t+1})\mid X_t}\big|\mid X_t}
%         \geq \nu_t\ell_t.
%     \end{align}
% \end{proof}


==> theorems/figures.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/directed-fastest-N3-r1.1.png} 
        % \caption{Generic} \label{fig:timing1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.65\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/directed-fastest-N4-r1.1.png} 
        % \caption{Competitors} \label{fig:timing2}
    \end{subfigure}

    % \caption{Some general caption of all the figures. In (\subref{fig:timing1}) you can see a  green square....}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/directed-slowest-N3-r1.1.png} 
        % \caption{Generic} \label{fig:timing1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/directed-slowest-N4-r1.1.png} 
        % \caption{Competitors} \label{fig:timing2}
    \end{subfigure}

    \vspace{1cm}
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/directed-slowest-N5-r1.1.png} 
        % \caption{Price regulation} \label{fig:timing3}
    \end{subfigure}
    \hfill
    % \begin{subfigure}[t]{0.45\textwidth}
    %     \includegraphics[width=0.5\linewidth]{pics/directed-slowest-N6-r1.1.png} 
    % \end{subfigure}
    % \caption{Some general caption of all the figures. In (\subref{fig:timing1}) you can see a  green square....}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/directed-oriented-fastest-N3-r1.1.png} 
        % \caption{Generic} \label{fig:timing1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/directed-oriented-fastest-N4-r1.1.png} 
        % \caption{Competitors} \label{fig:timing2}
    \end{subfigure}

    \vspace{1cm}
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/directed-oriented-fastest-N5-r1.1.png} 
        % \caption{Price regulation} \label{fig:timing3}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}[t]{0.5\textwidth}
    %     \includegraphics[width=1\linewidth]{pics/directed-orienteslowest-N6-r1.1.png} 
    % \end{subfigure}
    % \caption{Some general caption of all the figures. In (\subref{fig:timing1}) you can see a  green square....}
\end{figure}


\begin{figure}
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/directed-oriented-slowest-N3-r1.1.png} 
        % \caption{Generic} \label{fig:timing1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/directed-oriented-slowest-N4-r1.1.png} 
        % \caption{Competitors} \label{fig:timing2}
    \end{subfigure}

    \vspace{1cm}
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/directed-oriented-slowest-N5-r1.1.png} 
        % \caption{Price regulation} \label{fig:timing3}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}[t]{0.5\textwidth}
    %     \includegraphics[width=1\linewidth]{pics/directed-orienteslowest-N6-r1.1.png} 
    % \end{subfigure}
    % \caption{Some general caption of all the figures. In (\subref{fig:timing1}) you can see a  green square....}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/eulerian-slowest-N3-r1.1.png} 
        % \caption{Generic} \label{fig:timing1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/eulerian-slowest-N4-r1.1.png} 
        % \caption{Competitors} \label{fig:timing2}
    \end{subfigure}

    \vspace{1cm}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/eulerian-slowest-N5-r1.1.png} 
        % \caption{Price regulation} \label{fig:timing3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.45\textwidth}
        \includegraphics[width=1\linewidth]{pics/eulerian-slowest-N6-r1.1.png} 
    \end{subfigure}
    % \caption{Some general caption of all the figures. In (\subref{fig:timing1}) you can see a  green square....}
\end{figure}

\begin{figure}
    \centering

    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/eulerian-oriented-slowest-N3-r1.1.png} 
        % \caption{Generic} \label{fig:timing1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/eulerian-oriented-slowest-N4-r1.1.png} 
        % \caption{Competitors} \label{fig:timing2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/eulerian-oriented-slowest-N5-r1.1.png} 
        % \caption{Competitors} \label{fig:timing2}
    \end{subfigure}

    \vspace{1cm}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/eulerian-oriented-slowest-N6-r1.1.png} 
        % \caption{Generic} \label{fig:timing1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/eulerian-oriented-slowest-N7-r1.1.png} 
        % \caption{Competitors} \label{fig:timing2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{pics/eulerian-oriented-slowest-N8-r1.1.png} 
        % \caption{Competitors} \label{fig:timing2}
    \end{subfigure}
    % \caption{Some general caption of all the figures. In (\subref{fig:timing1}) you can see a  green square....}
\end{figure}
